Wearable Healthcare Devices for Monitoring Stress and Attention Level in Workplace Environments

Wearable devices have revolutionized healthcare monitoring, allowing us to track physiological conditions without disrupting daily routines. Whereas monitoring physical health and physical activities have been widely studied, their application and impact on mental health are significantly understudied. This work reviews the state-of-the-art, focusing on stress and concentration levels. These two can play an important role in workplace humanization. For instance, they can guide breaks in high-pressure workplaces, indicating when and how long to take. Those are important to avoid overwork and burn-out, harming employees and employers. To this end, it is necessary to study which sensors can accurately determine stress and attention levels, considering that they should not interfere with their activities and be comfortable to wear. From the software point of view, it is helpful to know the capabilities and performance of various algorithms, especially for uncontrolled workplace environments. This work aims to research, review, and compare commercially available non-intrusive measurement devices, which can be worn during the day and possibly integrated with healthcare systems for stress and concentration assessment. We analyze the performance of various algorithms used for stress and concentration level assessment and discuss future paths for reliable detection of these two parameters.

==> tables/ml_attention.tex <==

% \begin{table}[!ht]
% \centering
% \caption{Used ML algorithms for attention detection
% % , adapted from \cite{personalized_stress_monitoring}
%   }
%     \begin{bchart}[step=10, max=100, unit=\%]
%         \bcbar[text=SVM, value=90\% \cite{evaluation_of_learning} ,color=yellow!10]{90}
%             \smallskip
%         \bcbar[text=CNN-LSTM, value=89\% \cite{human_attention_recognition},color=purple!10]{89}
%             \smallskip
%         \bcbar[text=kNN, value=77\% \cite{classification_of_human} ,color=green!10]{77}
%             \smallskip
%         \bcbar[text=Ensemble, value=72\% \cite{classification_of_human} ,color=brown!10]{72}
%         \bcxlabel{Top attention detection accuracy}
%     \end{bchart}
% \label{table:ML_attention_chart}
% \end{table}

